Learning Semantically Coherent and Reusable Kernels in Convolution Neural Nets for Sentence Classification

The state-of-the-art CNN models give good performance on sentence classification tasks. The purpose of this work is to empirically study desirable properties such as semantic coherence, attention mechanism and reusability of CNNs in these tasks. Semantically coherent kernels are preferable as they are a lot more interpretable for explaining the decision of the learned CNN model. We observe that the learned kernels do not have semantic coherence. Motivated by this observation, we propose to learn kernels with semantic coherence using clustering scheme combined with Word2Vec representation and domain knowledge such as SentiWordNet. We suggest a technique to visualize attention mechanism of CNNs for decision explanation purpose. Reusable property enables kernels learned on one problem to be used in another problem. This helps in efficient learning as only a few additional domain specific filters may have to be learned. We demonstrate the efficacy of our core ideas of learning semantically coherent kernels and leveraging reusable kernels for efficient learning on several benchmark datasets. Experimental results show the usefulness of our approach by achieving performance close to the state-of-the-art methods but with semantic and reusable properties.

==> related_work1.tex <==
\section{Related Work}
CNNs have been very successful for image classification problems as they make use of internal structure of data such as the 2D structure of image data through convolution layers \cite{AK}. In the text domain, CNNs have been used for a variety of problems including sentence modeling, word embedding learning and sentiment analysis, by making use of 1D structure of document data.

More relevant to the work in this paper
is the work of \cite{kim2014convolutional}, where it was demonstrated that a simple CNN with one layer of convolution on top of static pre-trained word vectors, obtained using Word2Vec \cite{mikolov2013efficient}, achieved excellent results on sentiment analysis and question classification tasks. \cite{kim2014convolutional} also studied the use of multichannel representation and variable size filters.
\cite{kalchbrenner2014convolutional} proposed  Dynamic CNN (DCNN) that alternated wide convolutional layers with dynamic $k$-max pooling to model sentences.
%The network achieved good performance on question and sentiment %classification %data sets without requiring information provided by external resources %like word2vec.
\cite{Yin2} proposed Multichannel Variable-size CNN (MVCNN) architecture for sentence classification. It combines different versions of word embeddings and variable sized filters in a CNN with multiple layers of convolution.


\cite{le2014distributed} proposed an unsupervised framework that learns continuous distributed vector representations for variable-length pieces of texts, such as sentences or paragraphs.  The vector representations are learned to predict the surrounding context words sampled from the paragraph.
%The learned word and paragraph vectors are fed to a neural network with %a single hidden layer and logistic classifier for sentiment prediction.
The
focus is to learn paragraph vectors and task specific features are not taken into account.

\cite{genCNN} proposed an architecture, genCNN, to predict a word sequence by exploiting both long/short range dependencies present in the history of words. \cite{Johnson} compared the performance of two types of CNNs: seq-CNN in which every text region is represented by a fixed dimensional vector, and bow-CNN, which uses bag-of-word conversion in the convolution layer. %Experiments on sentiment classification data sets %showed that seq-CNN outperforms bow-CNN.

%Although \cite{kim2014convolutional} used multichannel convolution, the idea was %to use two copies of pre-trained Word2Vec embeddings: one was kept static and the %other was %trained. The success of MVCNN was mainly due to the idea of combining %different pre-trained word embeddings, the idea proposed by different %researchers \cite{Turian} and \cite{Luo}.

\cite{Zhang} applied CNNs only on characters and demonstrated that deep CNNs do not require the knowledge of words when trained on large-scale data sets. However, capturing semantic information using character-level CNNs is difficult.
%Although character-level CNNs do not require the knowledge %about the syntactic and semantic structure of a language when trained on %large data sets, interoperability of the designed CNN is an issue in this %case.
\cite{Santos} designed a Character to Sentence CNN (CharSCNN) that jointly uses character-level, word-level and sentence-level representations to perform sentiment analysis using two convolutional layers.
%to extract relevant features from words and sentences of any size.
%Effectiveness of CharSCNN was compared with RNTN (Recursive Neural Tensor
%Networks) \cite{socher2013recursive} for sentiment %analysis of sentences.

%When trying to answer a question about an image, one tends to focus attention on the informative regions according to question's intent. Based on this observation, attention based CNNs were proposed.
%\cite{ABC-CNN} proposed a attention based configurable CNN (ABC-CNN) for visual question answering task by using question guided attention region, located by a CNN, based on input queries. The attention regions are generated by a configurable CNN that is trained by the meaning of questions.
%\cite{Yin}
%came up with HABCNN that employs an attention mechanism to detect key phrases, sentences and snippets that are relevant to answering the question.
%Investigation on a Question-Answering benchmark data set showed that HABCNN outperforms prior deep learning approaches.

%Existing word embedding learning algorithms like word2vec typically ignore sentiment information of texts. This results in words such as good and bad, which indicate opposite sentiments, possibly getting mapped to neighbouring vectors.
%\cite{Tang} proposed a neural network to learn sentiment-specific word embeddings (SSWE) by capturing both the contexts of words and the sentiment information of sentences. The representation of words, thus obtained, are simply averaged to get a sentence representation. Use of a linear classifier on these representations demonstrated the usefulness of the proposed SSWE approach for twitter sentiment classification.

